MemFolder: Structure-Guided Memory Folding for Efficient Agent Memory Management

Long-term agents accumulate large external memory stores as interactions unfold, increasing the costs of storage, retrieval, and response generation. Efficiency is constrained by two coupled factors: a growing record count increases retrieval overhead, while longer retrieved contexts increase prefill computation and decoding-time attention costs. Existing methods prune or consolidate records, but pruning can discard useful evidence, whereas consolidation may produce fewer yet longer retrieval units. We introduce MemFolder, a structure-guided memory folding framework that sequentially reduces record count and context length. The framework comprises two core components that share memory groups, using cross-record structure to guide both evidence consolidation and compact representation. RecordFolder grounds entity mentions, progressively selects representative yet complementary anchors, and combines semantic and entity affinity with temporal chaining to consolidate compatible records into fewer retrieval units. ContextFolder encodes the original records within these groups into compact text and uses verification feedback to revise encodings when key facts cannot be recovered. Experiments on the three text-based memory benchmarks LoCoMo, PersonaMem, and LongMemEval and the two multimodal benchmarks M3-Bench-web and M3-Bench-robot demonstrate the strong performance of our methods. Notably, on Mem0, RecordFolder retains 99.0% of the original average performance across the three text-based benchmarks with 50% fewer records, exceeding the strongest baseline by 1.9 percentage points in performance retention. Combined with ContextFolder, existing record compression methods further shorten their output records while retaining most of their performance.

==> Tables/ablation_context.tex <==
\begin{table}[t]
\centering
\begin{minipage}{0.48\linewidth}
\centering
\caption{\textbf{Temporal chaining and consolidation: gain gating and global matching at $\kappa=0.5$.}}
\vspace{-3pt}
\fontsize{7}{10}\selectfont
\setlength{\tabcolsep}{1.2pt}
\setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{-10pt}
\begin{tabular}{l|cc|c|c}
\toprule[1.2pt]
\textbf{Assignment} & \textbf{LoCoMo} & \textbf{LongMemEval} & \textbf{Avg.} & \textbf{\%} \\
\midrule
w/o gain gate $g>0$      & 57.6 & 53.0 & 55.3 & 96.7\% \\
w/o temporal chaining    & 59.1 & 54.2 & 56.7 & 99.1\% \\
Greedy edges (no match)  & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} \\
Pairwise merge order     & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} \\
\rowcolor{memyellow}
\textbf{Hungarian (ours)} & \textbf{59.3} & \textbf{55.0} & \textbf{57.2} & \textbf{100.0\%} \\
\bottomrule[1.2pt]
\end{tabular}
\label{tab:chain}
\end{minipage}
\hspace{0.01\linewidth}
\begin{minipage}{0.48\linewidth}
\centering
\caption{\textbf{ContextFolder: planner, budgeted grammar and blind verification at $\kappa=0.5$.}}
\vspace{-3pt}
\fontsize{7}{10}\selectfont
\setlength{\tabcolsep}{1.2pt}
\setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{-10pt}
\begin{tabular}{l|cc|c|c}
\toprule[1.2pt]
\textbf{Encoding} & \textbf{Acc.} & \textbf{Tok./unit} & \textbf{Retr.} & \textbf{\%} \\
\midrule
w/o ContextFolder        & 59.3 & 20.6 & \textcolor{gray}{--} & \textcolor{gray}{--} \\
LLM summarize to $\tau$  & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} \\
w/o planner triage       & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} \\
w/o grammar (free prose) & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} \\
w/o verifier             & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{--} \\
\rowcolor{memyellow}
\textbf{MemFolder (full)} & \textbf{56.4} & \textbf{12.3} & \textbf{696} & \textbf{--} \\
\bottomrule[1.2pt]
\end{tabular}
\label{tab:contextfolder}
\end{minipage}
\end{table}

==> Tables/ablation_ratio.tex <==
\begin{table}[t]
    \caption{
    \textbf{Component necessity emerges as the record budget tightens.}
    Change in benchmark-averaged accuracy when one component of RecordFolder is removed.
    }
    \label{tab:ablation_ratio}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{14pt}
    \renewcommand{\arraystretch}{1.05}
    \begin{tabular}{lccc}
    \toprule
    \textbf{Removed component} & $\kappa\!=\!0.7$ & $\kappa\!=\!0.5$ & $\kappa\!=\!0.3$ \\
    \midrule
    \multicolumn{4}{l}{\textit{Anchor selection}} \\
    \hspace{7pt}Consolidation (prune only)  & --1.89 & --6.03 & --17.43 \\
    \hspace{7pt}Progressive order (random)  & --1.05 & --2.32 & --2.04 \\
    \midrule
    \multicolumn{4}{l}{\textit{Affinity and chaining}} \\
    \hspace{7pt}Entity signal $s_{\mathrm{ent}}$ & --0.16 & --1.06 & --1.66 \\
    \hspace{7pt}Embedding signal $\cos$         & --1.88 & --3.37 & --2.16 \\
    \hspace{7pt}Gain gate $g\!>\!0$             & +0.39 & --1.88 & --1.90 \\
    \hspace{7pt}Temporal chaining              & --1.75 & --0.52 & --0.86 \\
    \midrule
    \rowcolor{memyellow}
    \textbf{MemFolder (Ours), Avg.} & 58.5 & 57.2 & 56.1 \\
    \bottomrule
    \end{tabular}
    \vspace{-4mm}
\end{table}
